InvDiff: Invariant Guidance for Bias Mitigation in Diffusion Models

As one of the most successful generative models, diffusion models have demonstrated remarkable efficacy in synthesizing high-quality images. These models learn the underlying high-dimensional data distribution in an unsupervised manner. Despite their success, diffusion models are highly data-driven and prone to inheriting the imbalances and biases present in real-world data. Some studies have attempted to address these issues by designing text prompts for known biases or using bias labels to construct unbiased data. While these methods have shown improved results, real-world scenarios often contain various unknown biases, and obtaining bias labels is particularly challenging. In this paper, we emphasize the necessity of mitigating bias in pre-trained diffusion models without relying on auxiliary bias annotations. To tackle this problem, we propose a framework, InvDiff, which aims to learn invariant semantic information for diffusion guidance. Specifically, we propose identifying underlying biases in the training data and designing a novel debiasing training objective. Then, we employ a lightweight trainable module that automatically preserves invariant semantic information and uses it to guide the diffusion model's sampling process toward unbiased outcomes simultaneously. Notably, we only need to learn a small number of parameters in the lightweight learnable module without altering the pre-trained diffusion model. Furthermore, we provide a theoretical guarantee that the implementation of InvDiff is equivalent to reducing the error upper bound of generalization. Extensive experimental results on three publicly available benchmarks demonstrate that InvDiff effectively reduces biases while maintaining the quality of image generation. Our code is available at https://github.com/Hundredl/InvDiff.

==> Pics/a_input_sample_baseline_fairdiff_celeba.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{Pics/fair-diff black.png}
        \caption{Prompt: a face of
a celebrity without blond hair}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[t]{0.4\linewidth}
\includegraphics[width=1\textwidth]{Pics/fair-diff blond.png}
        \centering
        \caption{Prompt: a face of
a celebrity without black hair}
    \end{subfigure}
    \caption{Samples from baseline Fair-Diffusion, trained on CelebA}
    \label{fig:samples_fairdiff_celeba}
    \Description{}
\end{figure*}

==> Pics/a_input_sample_baseline_fairdiff_fairness.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{Pics/fair-diff female.png}
        \caption{Prompt: a face
of a female}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[t]{0.4\linewidth}
\includegraphics[width=1\textwidth]{Pics/fair-diff male.png}
        \centering
        \caption{Prompt: a face
of a male}
    \end{subfigure}
    \caption{Samples from baseline Fair-Diffusion, trained on Fairface}
    \label{fig:samples_fairdiff_fairness}
    \Description{}
\end{figure*}

==> Pics/a_input_sample_baseline_tiw_celeba.tex <==
\begin{figure*}[ht]
    \centering
     \includegraphics[width=0.8\linewidth]{Pics/sample_tiw_celeba.png}
    
    \caption{Samples from baseline TIW, trained on CelebA}
    \label{fig:samples_baseline_tiw_celeba}
    \Description{}
\end{figure*}

==> Pics/a_input_sample_baseline_tiw_fairness.tex <==
\begin{figure*}[ht]
    \centering
     \includegraphics[width=0.8\linewidth]{Pics/sample_tiw_fairness.png}
    
    \caption{Samples from baseline TIW, trained on Fairface}
    \label{fig:samples_baseline_tiw_fairness}
    \Description{}
\end{figure*}

==> Pics/a_input_sample_ours_celeba.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{Pics/sample_celeb_blond.png}
        \caption{Prompt: a face of
a celebrity without blond hair}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[t]{0.4\linewidth}
\includegraphics[width=1\textwidth]{Pics/sample_celeb_black.png}
        \centering
        \caption{Prompt: a face of
a celebrity without black hair}
    \end{subfigure}
    \caption{Samples from \shortname, trained on CelebA}
    \caption{}
    \label{fig:samples_invdiff_celeba}
    \Description{}
\end{figure*}

==> Pics/a_input_sample_ours_fairness.tex <==
\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=1\textwidth]{Pics/sample_fairness_female.png}
        \caption{Prompt: a face
of a female}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[t]{0.4\linewidth}
\includegraphics[width=1\textwidth]{Pics/sample_fairness_male.png}
        \centering
        \caption{Prompt: a face
of a male}
    \end{subfigure}
    \caption{Samples from \shortname, trained on Fairface}
    \label{fig:samples_invdiff_fairness}
    \Description{}
\end{figure*}

==> Pics/exp_delta_ratio.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Pics/Bias_CLIP-T.pdf}
        \caption{bias}
        \label{fig:exp_delta_ratio_bias}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
\includegraphics[width=\textwidth]{Pics/Recall_Precision.pdf}
        \caption{recall}
        \label{fig:exp_delta_ratio_recall}
    \end{subfigure}
     \caption{Impact of different $\Delta$ on model performance for the Waterbirds dataset}
    \label{fig:exp_delta_ratio}
    \Description{}
\end{figure}

==> Sections/author-names.tex <==

%\author{Anonymous Author(s)}
\iffalse
\author{%
  Min Hou\textsuperscript{\rm 1}\footnotemark[1], Yueying Wu\textsuperscript{\rm 2}\footnotemark[1], Chang Xu\textsuperscript{\rm 3}\footnotemark[2], Yu-Hao Huang\textsuperscript{\rm 4}, Chenxi Bai\textsuperscript{\rm 1}, Le Wu\textsuperscript{\rm 1},
  Jiang Bian\textsuperscript{\rm 3}\\
  \textsuperscript{\rm 1}Hefei University of Technology\ \
  \textsuperscript{\rm 2}Peking University\\
  \textsuperscript{\rm 3}Microsoft Research Asia\ \ \textsuperscript{\rm 4}Nanjing University\\
  \texttt{\{hmhoumin, chenxibai1149, lewu.ustc\}@gmail.com}\\
  \texttt{wuyueying@stu.pku.edu.cn, \{chanx, jiang.bian\}@microsoft.com}\\
  \texttt{huangyh@smail.nju.edu.cn}
}
\fi


\author{Min Hou}
\authornote{Both authors contributed equally to this research.}
\email{hmhoumin@gmail.com}
\affiliation{%
  \institution{Hefei University of Technology}
  \city{Hefei}
  \country{China}
}

\author{Yueying Wu}
\authornotemark[1]
\email{wuyueying@stu.pku.edu.cn}
\affiliation{%
  \institution{Peking University}
    \city{Beijing}
  \country{China}}

\author{Chang Xu}
\email{chanx@microsoft.com}
\affiliation{%
  \institution{Microsoft Research Asia}
    \city{Beijing}
  \country{China}
}

\author{Yu-Hao Huang}
\email{huangyh@smail.nju.edu.cn}
\affiliation{%
  \institution{Nanjing University}
    \city{Nanjing}
  \country{China}}

\author{Chenxi Bai}
\email{chenxibai1149@gmail.com}
\affiliation{%
  \institution{Hefei University of Technology}
  \city{Hefei}
  \country{China}
}

\author{Le Wu}
\email{lewu.ustc@gmail.com}
\affiliation{%
  \institution{Hefei University of Technology}  
  \city{Hefei}
  \country{China}
}

\author{Jiang Bian}
\email{jiang.bian@microsoft.com}
\affiliation{%
  \institution{Microsoft Research Asia}
  \city{Beijing}
  \country{China}
}


==> Tables/a_table_softgrouper.tex <==

\begin{table*}[!htbp]
\small
    \caption{Effect of  softgrouper}
    \label{tab:tab_softgrouper}
    \centering
    \begin{tabular}{c|cccc|cccc}
    \toprule
     & \multicolumn{4}{c|}{4group} & \multicolumn{4}{c}{8group} \\  
     \midrule
     Parameter Quantity of $\boldsymbol{G}_\psi$& FID $\downarrow$& Rec $\uparrow$& Bias$\downarrow$& CLIP-T $\uparrow$& FID $\downarrow$& Rec $\uparrow$& Bias$\downarrow$& CLIP-T $\uparrow$\\ 
     \midrule
     W0& 101.70& 0.59& 0.80(0.06)& 25.57(2.58)& 110.42& 0.49& 0.71(0.18)& 25.50(2.58)\\ 
     W3& 103.84&0.54& 0.79(0.12)& 25.45(2.61)& 114.23& 0.49& 0.75(0.15)& 25.04(2.69)\\ 
     W5& 115.77& 0.41& 0.72(0.16)& 25.25(2.75)& 108.55& 0.56& 0.70(0.20)& 25.22(2.64)\\
    \bottomrule
    \end{tabular}
\end{table*}

==> Tables/delta_param.tex <==

\begin{table*}[!htbp]
    \centering
    \caption{Impact of delta parameter quantity on model performance under different parameter settings}
    \resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc}
    \toprule
     & \multicolumn{4}{c|}{$\Delta$=0.2} & \multicolumn{4}{c}{$\Delta$=0.3} \\  
     \midrule
     Parameter Quantity of $\boldsymbol{G}_\psi$& Rec $\uparrow$ & Prec $\uparrow$ & Bias $\downarrow$ & CLIP-T $\uparrow$ & Rec $\uparrow$ & Prec $\uparrow$ & Bias $\downarrow$ & CLIP-T $\uparrow$\\ 
     \midrule
     860M(Param0)& 0.12& 0.32& 0.71(0.38)& 32.44(1.99) & \textbf{0.19}& 0.33& 0.69(0.37)& 32.08(2.10)\\ 
     551M(Param1)&0.13 &0.33 & \textbf{0.55(0.36)}& 32.55(2.03)& 0.17& 0.32& 0.66(0.41)& 31.89(2.32)\\ 
     220M(Param2)& 0.20& 0.31& 0.67(0.37)& 32.56(2.02)& 0.00& \textbf{0.73}& \textbf{0.56(0.32)}& 23.35(3.03)\\ 
     56M(Param3)& 0.17& 0.32& 0.72(0.36)& 32.72(1.91)& 0.07& 0.29& 0.67(0.37)& 32.59(1.95)\\ 
     15M(Param4)& \textbf{0.25}& \textbf{0.35}& 0.65(0.40)& \textbf{32.77(2.07)}& 0.05& 0.45& 0.76(0.38)& \textbf{32.67(1.94)}\\ 
     \bottomrule
    \end{tabular}}
\label{tab:exp_delta_param} 
\end{table*}

  

==> Tables/grouper.tex <==

\begin{table*}[!htbp]
\caption{Impact of grouper on model performance for the Waterbirds dataset}
    \label{tab:exp_grouper}
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{c|c|cccc|cccc}
    \toprule
    \multirow{2}{*}{} & & \multicolumn{4}{c|}{$\Delta$=0.2} & \multicolumn{4}{c}{$\Delta$=0.3} \\ \cmidrule(l){3-6} \cmidrule(l){7-10}
    & Grouper & Rec $\uparrow$ & Prec $\uparrow$ & Bias $\downarrow$ & CLIP-T $\uparrow$& Rec $\uparrow$ & Prec $\uparrow$ & Bias $\downarrow$ & CLIP-T $\uparrow$\\ \midrule
    \multirow{5}{*}{220M(Param2)} & Handcrafted & \textbf{0.20} & 0.31 & 0.67(0.37) & 32.56(2.02) & 0.00 & \textbf{0.73} & \underline{0.56(0.32)} & 23.35(3.03) \\ 
    & G2-Optimized & 0.13 & \textbf{0.36} & 0.57(0.29) & \underline{33.25(1.97)} & \textbf{0.18} & 0.33 & 0.63(0.31) & \textbf{32.86(2.17)} \\ 
    & G2-Balanced & 0.17 & 0.35 & \underline{0.51(0.30)} & 32.83(2.02) & \underline{0.11} & 0.44 & \textbf{0.54(0.31)} & \underline{32.70(2.00)} \\ 
    & G4-Optimized & \underline{0.19} & 0.35 & 0.66(0.33) & \textbf{33.22(2.01)} & 0.07 & 0.32 & 0.58(0.32) & 32.65(2.12) \\ 
    & G4-Balanced & \underline{0.19} & \textbf{0.36} & \textbf{0.46(0.34)} & 32.98(1.93) & 0.08 & \underline{0.48} & 0.59(0.27) & 32.48(2.11) \\ \midrule
    \multirow{5}{*}{56M(Param3)} & Handcrafted & \textbf{0.17} & 0.32 & 0.72(0.36) & \textbf{32.72(1.91)} & 0.07 & 0.29 & 0.67(0.37) & \textbf{32.59(1.95)} \\ 
    & G2-Optimized & 0.12 & \underline{0.44} & 0.69(0.31) & 32.54(1.97) & \textbf{0.16} & 0.44 & 0.70(0.29) & \underline{32.28(2.19)} \\ 
    & G2-Balanced & \underline{0.16} & 0.40 & \underline{0.67(0.25)} & 32.53(2.08) & 0.12 & \textbf{0.50} & 0.70(0.24) & 32.01(2.16) \\ 
    & G4-Optimized & \underline{0.16} & \textbf{0.46} & \textbf{0.55(0.27)}& 32.48(2.01) & 0.13 & \underline{0.49} & \textbf{0.54(0.31)} & 31.96(2.21) \\ 
    & G4-Balanced & 0.14 & 0.40 & 0.70(0.24) & \underline{32.70(1.99)} & \underline{0.14} & 0.48 & \underline{0.56(0.29)} & 31.98(2.16) \\ \bottomrule
    \end{tabular}}
    
\end{table*}

==> Tables/main.tex <==

\begin{table*}[!htbp]
\small
    \caption{Overall Image Generation Results.}
    \label{tab:exp_main}
    \centering
    \begin{tabular}{c|cccc|cccc}
    \toprule
     & \multicolumn{4}{c|}{Waterbirds} & \multicolumn{4}{c}{CelebA} \\  
     \midrule
     Model& Rec $\uparrow$ & Prec $\uparrow$ & Bias $\downarrow$ & CLIP-T $\uparrow$& Rec $\uparrow$ & Prec $\uparrow$ & Bias $\downarrow$ & CLIP-T $\uparrow$\\ 
     \midrule
     DPM& 0.15& 0.25& 0.89(0.25)& 31.59(2.03)& 0.34& 0.19& 0.75(0.24)& 25.27(1.35)\\ 
     DPM-G& 0.24&0.33& 0.85(0.25)& 30.84(2.31)& 0.39& 0.23& 0.58(0.41)& 25.41(1.37)\\ 
     \shortname & \textbf{0.25}& \textbf{0.35}& \textbf{0.65(0.40)}& \textbf{32.77(2.07)}& \textbf{0.48}& \textbf{0.25}& \textbf{0.57(0.42)}& \textbf{25.83(1.39)}\\
     \bottomrule
    \end{tabular}
\label{tab:main}
\end{table*}

==> Tables/searched_param.tex <==
\begin{table*}[!htbp]
    \centering
    \caption{Hyperparameters and candidate values for grid search}
    \label{tab:searched_param}
    \begin{tabular}{cc}
    \toprule
         Hyperparameters Name& Candidate Value\\
         \midrule
         batch size& \{8, 32, 64\}\\
         learning rate& \{1e-4, 1e-5\}\\
         lr scheduler & \{constant, linear, cosine, cosine with restarts, constant with warm up\}\\
         warm up step & \{0, 500, 1000\}\\
         parameter quantity of $\boldsymbol{G}_\psi$ & \{860M, 551M, 220M, 56M, 15M\}\\
         $\Delta$& \{0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.8, 0.9, 1, 2, 10\}\\
 $\lambda$&\{0.2, 0.4, 0.6, 0.8, 1, 2, 5, 10, 20, 50, 100\}\\
         \bottomrule
 
    \end{tabular}
    
\end{table*}

==> Tables/time_series_table1.tex <==
\begin{table*}[!ht]
\caption{{Comparison of $\text{CRPS}_{\text{sum}}$ (smaller is better) of models on six real-world datasets. The reported mean and standard error are obtained from 10 re-training and evaluation independent runs.}}
\label{tab-compare}
\resizebox{\textwidth}{!}{%
    \begin{tabular}{lllllllll}
    \toprule
    \multicolumn{1}{c}{\bfseries Method} & \multicolumn{1}{c}{\bfseries \texttt{Solar}}  &\multicolumn{1}{c}{\bfseries \texttt{Electricity}} &   \multicolumn{1}{c}{\bfseries \texttt{Traffic}}  &  \multicolumn{1}{c}{\bfseries \texttt{KDD-cup}} & \multicolumn{1}{c}{\bfseries \texttt{Taxi}} & \multicolumn{1}{c}{\bfseries \texttt{Wikipedia}}  \\ 
    \midrule
    Vec-LSTM ind-scaling & $0.4825_{\pm 0.0027}$ & $0.0949_{\pm 0.0175}$ & $0.0915_{\pm 0.0197}$  & $0.3560_{\pm 0.1667}$ &  $0.4794_{\pm 0.0343}$& $0.1254_{\pm 0.0174}$\\
    GP-Scaling& $0.3802_{\pm 0.0052}$ & $0.0499_{\pm 0.0031}$ & $0.0753_{\pm 0.0152}$ & $0.2983_{\pm 0.0448}$ & $0.2265_{\pm 0.0210}$ & $0.1351_{\pm 0.0612}$ & \\
    GP-Copula & $0.3612_{\pm 0.0035}$ & $0.0287_{\pm 0.0005}$ & $0.0618_{\pm 0.0018}$ & $0.3157_{\pm 0.0462}$ & $0.1894_{\pm 0.0087}$ & $0.0669_{\pm 0.0009}$  \\ 
    LSTM-MAF  & $0.3427_{\pm 0.0082}$ & $0.0312_{\pm 0.0046}$ & $0.0526_{\pm 0.0021}$ & $0.2919_{\pm 0.1486}$ & $0.2295_{\pm 0.0082}$ & $0.0763_{\pm 0.0051}$ \\
    Transformer-MAF  & $0.3532_{\pm 0.0053}$ & $0.0272_{\pm 0.0017}$ & $0.0499_{\pm 0.0011}$ & $0.2951_{\pm 0.0504}$ & $0.1531_{\pm 0.0038}$ &${0.0644}_{\pm 0.0037}$ \\
    TimeGrad & $0.3335_{\pm 0.0653}$ & $0.0232_{\pm 0.0035}$ & $0.0414_{\pm 0.0112}$ & $0.2902_{\pm 0.2178}$ & $0.1255_{\pm 0.0207}$ & $0.0555_{\pm 0.0088}$\\
  

    TACTiS & $0.4209_{\pm 0.0330}$ & $0.0259_{\pm 0.0019}$ & $0.1093_{\pm 0.0076}$ & $0.5406_{\pm 0.1584}$ & $0.2070_{\pm 0.0159}$& $-$ \\  
    % MG-Input & $0.3239_{\pm 0.0427}$  &  $0.0238_{\pm 0.0035}$ & $0.0658_{\pm 0.0065}$ & $0.2977_{\pm 0.1163}$ &  $0.1592_{\pm 0.0087}$ & $0.0567_{\pm 0.0091}$\\
    \shortname & $\bm{0.3121_{\pm 0.0087}}$ & $\bm{{0.0152}_{\pm 0.0019}}$ & $\bm{0.0382_{\pm 0.0134}}$ & $\bm{{0.2035}_{\pm 0.0854}}$ & $\bm{0.1344_{\pm 0.0253}}$ & $\bm{0.0549}_{\pm 0.0042}$\\
    \bottomrule
    \end{tabular}%
}
\end{table*}

